Tuning Pythia for Forward Physics Experiments

Event generators like Pythia play an important role in physics studies at the Large Hadron Collider (LHC). While they make accurate predictions in the central region, i.e. at pseudorapidities $\eta<5$, a disagreement between Pythia and measurements in the forward region, $\eta>7$, has been observed. We introduce a dedicated forward physics tune for the Pythia event generator to be used for forward physics studies at the LHC, which uses a more flexible modelling of beam remnant hadronization and is tuned to available particle spectra measured by LHCf. Furthermore, we provide an uncertainty estimate on the new tune in a data-driven way which can be used as a means of flux uncertainty for future forward physics studies. We demonstrate an application of our tune by showing the updated neutrino and dark photon spectra at the FASER experiment.

==> header.tex <==

\RequirePackage[colorlinks=true
,urlcolor=blue
,anchorcolor=blue
,citecolor=blue
,filecolor=blue
,linkcolor=blue
,menucolor=blue
,linktocpage=true
,pdfproducer=medialab
,pdfa=true
]{hyperref}

\usepackage{amsmath,amssymb,amsthm,amsfonts}
\usepackage{graphicx,tabularx}
\usepackage{color}
\usepackage{multirow}
\usepackage{comment}
\usepackage{enumitem}
\usepackage{cleveref}
\usepackage{soul}
\usepackage{slashed}
\usepackage[normalem]{ulem}
\usepackage{scalerel}
\usepackage{wrapfig}
\usepackage{cancel}
\usepackage{xcolor}
%\usepackage{todonotes}
\usepackage{titlesec}
\usepackage[letterpaper,dvips,hmargin={1in,1in},vmargin={1in,1in}]{geometry}

\titlespacing*{\subsection}{0pt}{\baselineskip}{\baselineskip}

\setlist[description]{leftmargin=0.3cm}
\setlist[itemize]{leftmargin=0.5cm}

\newcommand{\be}{\begin{equation} \begin{aligned}}
\newcommand{\ee}{\end{aligned} \end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}

\def\figureautorefname~#1\null{Fig.\,#1\null}
\def\tableautorefname~#1\null{Tab.\,#1\null}
\renewcommand{\sectionautorefname}{Sec.}
\renewcommand{\subsectionautorefname}{Sec.}
\def\equationautorefname~#1\null{Eq.\,(#1)\null}

% General symbols
\newcommand{\im}{\mathrm{i}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\eg}{{e.\,g.}~}
\newcommand{\ie}{{i.\,e.}~}
\newcommand{\equivalent}{\simeq}
\newcommand{\br}{\mathrm{BR}}

% Units
\newcommand{\ev}{\text{eV}}
\newcommand{\kev}{\text{keV}}
\newcommand{\mev}{\text{MeV}}
\newcommand{\gev}{\text{GeV}}
\newcommand{\tev}{\text{TeV}}

\newcommand{\ab}{\text{ab}}
\newcommand{\iab}{\text{ab}^{-1}}
\newcommand{\fb}{\text{fb}}
\newcommand{\ifb}{\text{fb}^{-1}}
\newcommand{\pb}{\text{pb}}
\newcommand{\ipb}{\text{pb}^{-1}}

\newcommand{\nm}{\text{nm}}
\newcommand{\micm}{\mu\text{m}}
\newcommand{\mm}{\text{mm}}
\newcommand{\cm}{\text{cm}}
\newcommand{\m}{\text{m}}
\newcommand{\km}{\text{km}}

\newcommand{\mrad}{\text{mrad}}
\newcommand{\murad}{\mu\text{rad}}

\newcommand{\g}{\text{g}}
\newcommand{\kg}{\text{kg}}
\newcommand{\ton}{\text{t}}
\newcommand{\sr}{\text{sr}}
\newcommand{\ns}{\text{ns}}
\newcommand{\hz}{\text{Hz}}

\newcommand{\fasernu}{FASER$\nu$~}

\newcommand{\sibyll}{\textsc{Sibyll}~}
\newcommand{\eposlhc}{\textsc{Epos-Lhc}~}
\newcommand{\qgsjet}{\textsc{QgsJet}~}
\newcommand{\pythia}{\textsc{Pythia}~}
\newcommand{\sibyllfs}{\textsc{Sibyll}}
\newcommand{\eposlhcfs}{\textsc{Epos-Lhc}}
\newcommand{\qgsjetfs}{\textsc{QgsJet}}
\newcommand{\pythiafs}{\textsc{Pythia}}


\newcommand{\rivet}{\textsc{Rivet}~}

\newcommand{\pT}{p_{\perp}}
\newcommand{\kT}{k_{\perp}}
\newcommand{\qbar}{\overline{q}}

\newcommand{\Eqref}[1]{Equation~(\ref{eq:#1})}
\newcommand{\Eqsref}[2]{Equations~(\ref{eq:#1}) and (\ref{eq:#2})}
\renewcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\eqsref}[2]{Eqs.~(\ref{eq:#1}) and (\ref{eq:#2})}
\newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\secsref}[2]{Secs.~\ref{sec:#1} and \ref{sec:#2}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\Secsref}[2]{Sections~\ref{sec:#1} and \ref{sec:#2}}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\figsref}[2]{Figs.~\ref{fig:#1} and \ref{fig:#2}}
\newcommand{\figssref}[3]{Figs.~\ref{fig:#1}, \ref{fig:#2} and \ref{fig:#3}}
\newcommand{\Figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tableref}[1]{Table~\ref{table:#1}}
\newcommand{\tablesref}[2]{Tables~\ref{table:#1} and \ref{table:#2}}
\newcommand{\appref}[1]{Appendix~\ref{sec:#1}}
\newcommand{\appsref}[2]{Appendices~\ref{sec:#1} and \ref{sec:#2}}


%comments
\RequirePackage[normalem]{ulem} 
\newcommand{\changed}[2]{{\protect\color{red}\sout{#1}}{\protect\color{blue}\uwave{#2}}}
%\newcommand{\changed}[2]{#2}

%\newcommand{\rem}[1]{}
\crefname{section}{Sec.}{Secs.}
\crefname{figure}{Fig.}{Figs.}
\crefname{equation}{Eq.}{Eqs.}
\crefname{table}{Table}{Tables}
\crefname{appendix}{Appendix}{Appendices}

% space on top/bottom from figures (copied from revtex)
\setcounter{topnumber}{2}
\def\topfraction{1}
\setcounter{bottomnumber}{1}
\def\bottomfraction{1}
\setcounter{totalnumber}{3}
\def\textfraction{0}
\def\floatpagefraction{1}
\setcounter{dbltopnumber}{2}
\def\dbltopfraction{1}
\def\dblfloatpagefraction{1}

%Ref Style
\bibliographystyle{utphys}

\crefname{appendix}{Appendix}{Appendices}
\makeatletter
\def\l@subsubsection#1#2{}
\makeatother

% by max
\usepackage{soul}
\usepackage[T1]{fontenc}
\usepackage{lmodern}
\usepackage{csvsimple}
\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage{centernot}
\usepackage{booktabs} % To thicken table lines

%\DeclareRobustCommand{\hlgre}[1]{{\sethlcolor{green}\hl{#1}}}
%\DeclareRobustCommand{\hlred}[1]{{\sethlcolor{red}\hl{#1}}}
%\DeclareRobustCommand{\hlora}[1]{{\sethlcolor{orange}\hl{#1}}}

% Personal Comments
\newcommand{\Felix}[1]{\textcolor{magenta}{[FK: #1]}}
\newcommand{\mf}[1]{\textcolor{blue}{[MF: #1]} }


\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.1}


